Higgs Pair Production: Choosing Benchmarks With Cluster Analysis

New physics theories often depend on a large number of free parameters. The precise values of those parameters in some cases drastically affect the resulting phenomenology of fundamental physics processes, while in others finite variations can leave it basically invariant at the level of detail experimentally accessible. When designing a strategy for the analysis of experimental data in the search for a signal predicted by a new physics model, it appears advantageous to categorize the parameter space describing the model according to the corresponding kinematical features of the final state. A multi-dimensional test statistic can be used to gauge the degree of similarity in the kinematics of different models; a clustering algorithm using that metric may then allow the division of the space into homogeneous regions, each of which can be successfully represented by a benchmark point. Searches targeting those benchmark points are then guaranteed to be sensitive to a large area of the parameter space. In this document we show a practical implementation of the above strategy for the study of non-resonant production of Higgs boson pairs in the context of extensions of the standard model with anomalous couplings of the Higgs bosons. A non-standard value of those couplings may significantly enhance the Higgs pair production cross section, such that the process could be detectable with the data that the Large Hadron Collider will collect in Run 2.

==> sec-intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%
\vskip .3cm

After the Run 1 discovery of a new scalar particle at 125 GeV~\cite{higgsdiscoveryAtlas,Chatrchyan:2012ufa} the LHC experiments are now looking forward to the data they are collecting in Run 2 and in the higher-luminosity phases that will follow. New discoveries are possible with the significantly increased centre-of-mass energy of proton-proton ({\em pp}) collisions and the foreseen integrated luminosity. The new data will also enable a deep investigation of the 125 GeV particle.

The standard model (SM) Lagrangian for the Higgs doublet contains a quartic scalar interaction,
the term which, together with the negative sign mass term $-\mu^2$, drives electroweak symmetry breaking (EWSB) (see however~\cite{Goertz:2015dba}). Moreover, one additional physical state, the Higgs boson {\em h}~\footnote{In this article we follow the terminology which has become standard in high-energy physics, namely we call ``Higgs boson'' the scalar particle resulting from the Brout-Englert-Higgs (BEH) mechanism when adding a complex doublet of scalar fields to the unbroken standard model Lagrangian.},  emerges in the theory, with cubic and quartic self couplings resulting from the quartic interaction of the scalar doublet. In the SM scenario the strength of all Higgs boson couplings is precisely predicted; deviations from those predictions would thus imply the existence of beyond-standard-model (BSM) physics. A high-statistics study of the couplings of the newly discovered boson may therefore reveal whether we are in the presence of the last building block of the SM, or rather of the first one of a new physics sector.

The idea of probing BSM physics scenarios (especially the Higgs trilinear coupling) in non-resonant Higgs boson pair production at proton-proton colliders dates far before the top quark discovery and the LHC design~\cite{Glover:1987nx}; a large number of studies have been performed since then. After the Higgs boson discovery, many authors have investigated different phenomenological aspects of the topic (see for example~\cite{
Dawson:2015oha,Azatov:2015oxa,  Slawinska:2014vpa, Barger:2013jfa, Barr:2014sga, Liu:2014rba, Goertz:2014qta, Chen:2014xra, Dolan:2012ac, Goertz:2013kp,  Nishiwaki:2013cma, Yao:2013ika,Shao:2013bz,Wardrope:2014kya,Dolan:2015zja,He:2015spf,Dolan:2015zja,Lu:2015jza, Cao:2013si,Cao:2014kya,Papaefstathiou:2015iba,deLima:2014dta,Maierhofer:2013sha,Papaefstathiou:2012qe}); most of the phenomenology-driven works have focused on the effects of a variation of the Higgs boson trilinear coupling $\lambda$.  
In the present work we consider that any kind of coupling deviation from the SM Higgs sector is a proof that the SM is not complete; therefore {\em all} possible Higgs boson couplings should be considered as ingredients of a BSM extension of the standard model~\footnote{It is interesting to note that by measuring Higgs boson pair production, one can even probe the very presence of the $\mu^2$ term, {\em i.e.} the relevant $H^2$ operator (before electroweak symmetry breaking)~\cite{Goertz:2015dba}.}.
The parameter space resulting from that interpretation is multi-dimensional; its systematic study calls for a principled approach, which we aim to provide here. In this paper we will focus on gluon-gluon fusion (GF) production of Higgs boson pairs, which is the simplest process available to probe the Higgs boson self-coupling at the LHC. The possible BSM deviations in inclusive di-Higgs production arising in other production modes, such as vector-boson fusion~\cite{Hankele:2006ma,VBFhh} or associated production with top quarks (see for example~\cite{Englert:2014uqa,Liu:2014rva}) or vector bosons, probe a different set of parameters in the context of an effective-field theory (EFT) as the one we are considering. The interpretation of the results of those channels should be studied separately. 

Measurements performed by the ATLAS and CMS collaborations with Run 1 LHC data have already started to constrain the value of some of the Higgs boson couplings~\cite{Khachatryan:2014jba, ATLAS-CONF-2015-007}. Due to interference effects, even small modifications of some of the couplings within the constraints posed by measurements may change drastically the di-Higgs signal topology, and enhance the production cross section enough to make the process accessible with Run 2 data. For that to happen, the observable features of the final state need to be exploited in an optimized way, given the huge cross section of physical processes yielding irreducible backgrounds. This implies making full use of the distinguishing characteristics of signal events in the multi-dimensional space of their observable features. What is needed is therefore the identification of a manageably small set of benchmark points which are maximally representative of the largest possible volume of the unexplored parameter space. The investigation of those points in as much detail as possible will effectively provide information on the full model space. 

We employ a very general parametrization to sample the di-Higgs signal topology, assuming the absence of new heavy particles accessible at the LHC energy, which can for example describe the effects of strongly-coupled BSM theories (without being limited to those); we provide it in Sec.~\ref{sec:lag}. The rest of this work is organized as follows: in Sec.~\ref{sec:cluster} we describe in detail the technique we devised to determine the similarity of final state densities in the space of observable kinematics, and the clustering procedure which uses that measure of similarity to identify homogeneous regions in the parameter space. In Sec.~\ref{sec:res} we describe the application of the technique to determine optimal benchmarks for the study of anomalous di-Higgs boson production, and we discuss the special features of the resulting partition of the parameter space. We finally draw some conclusions in Sec.~\ref{sec:conclu}. In the Appendix we also provide the coefficients of our parametrization of the di-Higgs production cross section.


==> sec-th.tex <==
\section{Sampling Signal Kinematics in the Higgs Couplings Basis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:lag}
\vskip .3cm

In the SM, Higgs boson couplings are exclusively controlled by the particle masses; couplings to light quarks are negligible. Higgs pair production occurs predominantly by gluon-gluon fusion (GF) via an internal fermion loop, where the top quark contribution is dominant. The extension of this assumption to BSM theories is well motivated if the Higgs sector is minimal (see also \cite{Goertz:2014qia}).  
%with five parameters controlling its tree-level interactions relevant for di-Higgs production. Written in terms of physical states as in equation~\ref{eq:lag}
In the absence of new light states, the GF Higgs pair production at the LHC can be generally described (to leading approximation) by five parameters controlling tree-level interactions of the Higgs boson. These five parameters are $\kappa_{\lambda}$, $\kappa_{t}$, $c_g$, $c_{2g}$, and $c_2$. The Higgs boson trilinear coupling and the top Yukawa interaction do exist in the SM Lagrangian, where the former is given by $\lambda_{SM}=m_h^2/2v^2$, with $v$ the vacuum-expectation value of the Higgs field. Deviations from SM values are parametrized with the multiplicative factors $\kappa_{\lambda}$ and $\kappa_{t}$, respectively. The contact interactions of the Higgs boson with gluons and those coupling two Higgs bosons with two gluons or a top-antitop quark pair, which could arise through the mediation of very heavy new states, are instead genuinely not predicted by the SM; they can be parametrized by the absolute couplings $c_g$, $c_{2g}$, and $c_2$. The Lagrangian then takes the form \par

\begin{eqnarray}
{\cal L}_h = 
\frac{1}{2} \partial_{\mu}\, h \partial^{\mu} h - \frac{1}{2} m_h^2 h^2 -
  {\kappa_{\lambda}}\,  \lambda_{SM} v\, h^3 
- \frac{ m_t}{v}(v+   {\kappa_t} \,   h  +  \frac{c_{2}}{v}   \, h\,  h ) \,( \bar{t_L}t_R + h.c.) \nonumber  \\ 
+ \frac{1}{4} \frac{\alpha_s}{3 \pi v} (   c_g \, h -  \frac{c_{2g}}{2 v} \, h\, h ) \,  G^{\mu \nu}G_{\mu\nu}\,.
\label{eq:lag}
\end{eqnarray}

\noindent
One should note that, in the case of a linear realization of electroweak symmetry breaking, we get $c_{2g} = - c_g$ within the EFT framework considered here, which describes the effects of new heavy states beyond present experimental reach via operators of dimension $4<D\leq6$ ~\cite{Giudice:2007fh,Buchmuller:1985jz,Contino:2013kra,Gillioz:2012se}~\footnote{Our normalization for the Higgs boson interaction with gluons is inspired by the infinite top-mass limit of the SM. The existence of a relative sign between $c_{2g}$ and  $c_g$ in this limit is a special feature of the SM, related to the chiral nature of SM fermions. }.
In Equation~\ref{eq:lag} we have assumed that Higgs boson couplings to light fermions are negligible, and the absence of any other light state in addition to the SM particles~\cite{Dawson:2015oha}\footnote{ In particular, in models with an extended (non-decoupling) Higgs sector, the coupling of the Higgs boson to bottom quarks might also be enhanced in the limit of large scalar mixing. The topology of double Higgs production would consequently be modified: besides the presence of a component of the signal initiated by bottom-antibottom quark fusion, the gluon-fusion topology would be modified since loop factors would now contain a non-negligible component with a low-mass quark~\cite{Plehn:1996wb}. An enhanced Higgs boson coupling to bottom quarks is not the only physical effect that could arise in Supersymmetric (SUSY) theories, where heavy SUSY scalars are predicted (see for example~\cite{Belyaev:1999kk,Spira:1997ce,Han:2013sga}). In the context of SUSY scenarios non-resonant di-Higgs production  is a wide topic, and we do not discuss it further in this document, although our treatment may still be useful in the decoupling limit, where all new states are heavy.}. In addition, we do not consider CP-violating BSM effects. Note in this context that for the potentially interesting case of the bottom 
quark Yukawa coupling $\kappa_b$, LHC data already constrains it within $0.75<\kappa_b<1.25$ \cite{Corbett:2015ksa} in the EFT, excluding large enhancements and justifying its omission as a good approximation. The different processes contributing to a di-Higgs signal in pp collisions at leading order (LO) are shown as Feynman diagrams in Figure~\ref{fig:dia}.

\begin{figure}[h]
\centering
\includegraphics[scale=0.85]{translation.pdf}
\caption{\small Feynman diagrams of processes that contribute to Higgs pair production by gluon-gluon fusion at leading order. Diagrams (a) and (b) correspond to SM-like processes, while diagrams (c), (d), and (e) corresponds to pure BSM effects: (c) and (d) describe contact interactions between the Higgs boson and gluons, and (e) exploits the contact interaction of two Higgs bosons with top quarks.   \label{fig:dia}}
\end{figure}

In Equation~\ref{eq:lag} we included operators with higher orders of the Higgs boson fields, which are for example a common feature of models where the Higgs doublet is a pseudo-Goldstone boson of a new strong symmetry and its effective interactions come from field expansions~\cite{Dugan:1984hq,Giudice:2007fh}. The translation of our parametrization to the flavour-diagonal Higgs basis (see~\cite{Falkowski:2014tna, Falkowski:2015fla}), which has been endorsed by the LHCHXSWG document~\cite{Duehrssen-Debling:2001958} as a general EFT basis to be used to derive experimental results, is trivial; for simplicity we prefer to keep the notation of Equation~\ref{eq:lag}. 
%%%%%%%%%%%%%%%% TO BE INCLUDED ONCE WE REINSTALL THE APPENDIX The correspondence between the coefficients in equation~\ref{eq.lag} with the notation that is currently being developed by the Higgs cross section working group~\cite{hxswg15} is provided in Appendix~(\ref{sec:basis}). 
%There is an analytical relation between the coefficients of the coupling basis (equation \ref{eq:lag}) with any dimension-6 EFT operators basis. 
Any dimension-6 EFT basis is related to the Higgs basis by analytical relations among the coefficients; the automation of basis conversions is under development~\cite{roseta}.  % with the Higgs doublet, . 
%We also included contact interactions of Higgs bosons with gluons, which may appear if very heavy colored particles mediate the gluon-Higgs interaction, which is tipically loop-suppressed. [TD- already said]

The differential cross section for the full process is proportional to the matrix element squared. Ideally, at any order of a radiatively corrected calculation we may write the square of the full matrix element (ME) as Equation~\ref{eq:ME}; the various terms in the matrix element expression contribute differently in different regions of the kinematic space:\par

\begin{eqnarray}
| M_{full}|^2 = 
 |M_{\lambda}|^2 + |M_{\Box}|^2 +  |M_{c_2}|^2 +  |M_{c_g}|^2 +  |M_{c_{2g}}|^2 + \nonumber \\   
 \, (M_{\lambda} M_{\Box}^{\dagger})  + 
  \, (M_{\lambda} M_{c_2}^{\dagger})  + 
   \, (M_{\lambda} M_{c_g}^{\dagger})  +  
    \, (M_{\lambda} M_{c_{2g}}^{\dagger}) + \nonumber \\ 
  \, (M_{\Box} M_{c_2}^{\dagger})  + 
   \, (M_{\Box} M_{c_g}^{\dagger})  + 
    \, (M_{\Box} M_{c_{2g}}^{\dagger})  + \nonumber \\
   \, (M_{c_2} M_{c_g}^{\dagger})  + 
    \, (M_{c_2} M_{c_{2g}}^{\dagger})  + 
    \, (M_{c_g} M_{c_{2g}}^{\dagger})  + \rm{ h.c}. \,.
    \label{eq:ME}
\end{eqnarray}
Above, $M_{j}$ identifies the matrix element piece where the parameter $j$ is the representative one, and $M_{\Box}$ corresponds to the box diagram.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cross Section and Parameter Space Study \label{sec:CX}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to carry out a phenomenological study we need to first define the range of parameter variations we are willing to consider. Some of the parameters relevant to the production phase are completely unconstrained by single Higgs boson measurements: among these are the triple Higgs coupling and the di-Higgs contact interactions with top quarks and gluons. Others, such as the top Yukawa coupling, are already constrained by experimental results~\cite{Khachatryan:2014jba, ATLAS-CONF-2015-007}. A precise interpretation of all experimental bounds on the effective operators and their effect on the considered process is not trivial, as the parameters do not only affect the predicted rate of di-Higgs production, but also the kinematics of the final state. 

Measurements of single Higgs boson production performed so far at the LHC already constrain the $\kappa_{t}$ and $c_g$ parameters. The combination of those results using the $\kappa$ formalism~\cite{Artoisenet:2013puc} shows that by marginalising over all other Higgs couplings the allowed values of $\kappa_{t}$ are constrained at $95\%$ C.L. in the region between 0.5 and 2.5. % of its standard value ($\kappa_{t}^{SM} =  1$). 
A Bayesian analysis of BSM operators based on available Higgs results constrains the $c_g$ parameter to be at most at the $O(1)$ level~\cite{Dumont:2013wma,Elias-Miro:2013mua,Pomarol:2013zra,Gupta:2014rxa,Corbett:2015ksa}. The remaining parameters are constrained only by absolute cross section limits on inclusive di-Higgs production~\cite{Aad:2014yja} as explained below.
The theoretical range of validity of the setup is to some extent model-dependent; for example it will depend on what is the actual scale of new physics setting the cut-off of the theory.
The full cross section of GF Higgs pair production can be expressed by a polynomial in terms of all the model parameters as in Equation~\ref{eq:cx}. 

\begin{eqnarray}
\frac{\sigma_{hh}}{\sigma_{hh}^{SM}} =   \left( 
\begin{matrix}
A_1\, \kappa_t ^4 + A_2\, c_2^2 + (A_3\, \kappa_t^2 + A_4\, c_g^2)\, \kappa_{\lambda}^2 
+ A_5\, c_{2g}^2 + ( A_6\, c_2 + A_7\, \kappa_t \kappa_{\lambda} )\kappa_t^2  \\
+ (A_8\, \kappa_t \kappa_{\lambda} + A_9\, c_g \kappa_{\lambda} ) c_{2} + A_{10}\, c_2 c_{2g} 
+ (A_{11}\, c_g \kappa_{\lambda} + A_{12}\, c_{2g})\, \kappa_t^2  \\
+ (A_{13}\, \kappa_{\lambda} c_g + A_{14}\, c_{2g} )\, \kappa_t \kappa_{\lambda} + A_{15}\, c_{g} c_{2g} \kappa_{\lambda} 
\end{matrix} 
\right)
\label{eq:cx}
\end{eqnarray}

\noindent
In proton-proton collisions at 13 TeV the prediction is $\sigma_{hh}^{SM} = 34.3 \mbox{ fb  }\pm 9\% \mbox{ (scale)} \pm 2\%$(PDF), while at 8 TeV it is $\sigma_{hh}^{SM} = 9.96 \mbox{ fb  } \pm 10\% \mbox{ (scale)}  \pm 2\%$ (PDF). Those values are based on recent progress~\cite{deFlorian:2014rta,Grigo:2014jma}, which use the {\tt CT10} PDF set~\cite{Gao:2013xoa} and employ as input the mass values $m_h = 126$ GeV, $m_t = 173.18$ GeV, and $m_b = 4.75$ GeV. 
%Regarding the dimension-six parametrization, relevant calculations are described in~\cite{Grober:2015cwa}. 
At LO the scattering amplitude for the $gg\to hh$ process contains terms with different loop structures, corresponding to the different BSM operators. 
%Therefore one can imagine that real jet emissions at next-to-leading order in QCD could yield significantly more complex topologies with respect to LO predictions.  The complications could depend on the microscopic nature of the interaction, i.e. on whether the matrix amplitude in a given parameter space point is dominated by box-like, by triangle-like, or by point-like interactions. 
The real emissions for the $gg\to hh$ process are not trivial to compute; the relative diagrams would contain up to pentagons to be matched with parton showers. 
Different groups of phenomenologists are progressing in the calculation of (N)NLO predictions matched to shower-level effects for the GF di-Higgs process, especially for the SM case; see for example~\cite{Maltoni:2014eza,Frederix:2014hta,Grigo:2015dia,deFlorian:2015moa,Grober:2015cwa}. 

The simulation setup used in this paper was produced by the authors of~\cite{Hespel:2014sla}. The LO process is already at one-loop level; in the approach followed in~\cite{Hespel:2014sla}, loop factors are calculated on an event-by-event basis with a {\tt Fortran} routine on top of an $aMC@NLO$~\cite{Frixione:2010ra, Alwall:2014hca} effective model; the {\tt NN23LO1} PDF set~\cite{Ball:2009mk} is used. Those simulations represent the state-of-the art in the description of BSM di-Higgs production. We simplify the task of mapping the five-dimensional parameter space of BSM theories in the limit of the present computational capability by assuming that each of the matrix element pieces of Equation~\ref{eq:ME} is equivalent to the use of an overall k-factor, as written in the first equality of Equation~\ref{eq:NNLO}. As a second step we make the stronger assumption that the k-factors related to the different ME pieces are equal, and that they may be taken as a k-factor derived for the SM case, leading to the second equality in Equation~\ref{eq:NNLO}:

\begin{equation}
 (M_{i} M_{j}^{\dagger} + h.c.)^{\mbox{\small higher order}} = k_{ij} \, (M_{i} M_{j}^{\dagger} + h.c.)^{(LO)}
 = k_{SM} \, (M_{i} M_{j}^{\dagger} + h.c.)^{(LO)}\,.
 \label{eq:NNLO}
\end{equation}

\noindent
The above approximations are expected to be good for QCD-like radiative corrections when
quoting the total cross section. Indeed, the enhancement in the total cross section from QCD NLO corrections is mainly due to soft gluon radiation from initial state~\cite{Grober:2015cwa}. For a characterization of the differential distributions, on the other hand, the description outlined above might not be entirely satisfactory. Bearing in mind that potential caveat, we decided to use it for this study as it facilitates the mapping of experimental results derived with LO simulations to the results of a radiative corrected calculation.

Using Equation~\ref{eq:NNLO} it is possible to calculate the coefficients of the polynomial in Equation~\ref{eq:cx} by  evaluating the results of LO computations in different points of the five-dimensional parameter space. For each considered point, using the setup mentioned above, we generate 20,000 pp collision events at 13 TeV centre of mass energy, producing a final state of two Higgs bosons. The resulting cross sections are then fit with a maximum likelihood technique to the polynomial~\ref{eq:cx}. 
In order to ensure a stable fit we inspect six orthogonal 2D planes in the 5-dimensional parameter space that contain the point corresponding to the SM. The procedure used to derive the coefficients of the polynomial in Equation~\ref{eq:cx} and the numerical results for the fitted parameters are detailed in~\cite{CarvalhoAntunesDeOliveira:2130724,}. Figure~\ref{fig:cx} shows the resulting cross section in the 2D planes mentioned above.

% ----------reimplement the below table once we have numbers!!
%We follow the cross section parametrization adopted by \cite{Lu:2015jza}, transcribed in Table~\ref{tab:cx13}.  
%The numbers were derived using a {\tt Herwig++} implementation of the  di-Higgs processes as implemented by the authors of \cite{andreas}, 
%and cross checked with the $aMC@NLO$ model implementation used to the kinematic study of this paper; see Appendix \ref{sec:coef} for details of the derivation. 

%\begin{table}[h]
%\centering
%\small{
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%%\multicolumn{3}{|c|}{$ \sigma_{0}^{NNLO} = XX$ pb (XX pb)  } \\[2mm]\hline
%$A_1$ = 2.2052 (28) & $A_4$ = 0.11671(14) & $A_7$ = -1.4646(22) & $A_{10}$ = -1.871(22) & $A_{13}$ = 0.3516(15) \\ 
%$A_2$ = 10.808(15) & $A_5$ = 1.4597(54) & $A_8$ = 2.922(13) & $A_{11}$ = -0.7356(36) & $A_{14}$ = -0.8995(47) \\ 
%$A_3$ = 0.30365(47) & $A_6$ = -8.925(0.023) & $A_9$ = -1.792(22) & $A_{12}$ = 2.0073(0.0064) & $A_{15}$ = -0.6315(45) \\ 
 %  \hline
%\end{tabular}
%}
%\caption{\small Coefficients of equation (\ref{eq:cx}) for LHC proton-proton collisions at 13 TeV. % following \cite{Lu:2015jza}. 
%\label{tab:cx13}} %TABLE TO DO!!!!!!!!!!!!!! }
%\end{table} 

%----------------------

%, for this purpose we may use the most recent value of cross section for the SM from the literature. %Following recent recommendations~\cite{hcxwg}, 
%We use the parameter space grid described in the previous subsection to calculate the coefficients of equation (\ref{eq:cx}) for the LHC at 13 TeV. We also derive the same coefficients for 8 TeV collisions using 162 samples simulated with the same setup. 

% Results can be found in table (\ref{tab:cx13}). 
%%%%%We find XXXXX\% agreement with reference \cite{Azatov:2015oxa} what is expected inside QCD uncertainties {\bf WORK TO DO!!!!!!!!!!!!!!}. 
%%% Until we have the number better leave this sentence off 
%The Higgs boson has a narrow width, as predicted by theory and indirectly measured~\cite{Khachatryan:2014iha,ATLAS}; therefore, investigations about its production and decay can be factorized. We estimate the bounds in parameter space assuming SM-like branching fractions of the Higgs boson.  
%%%%% Did not understand previous sentence - TD
 
\begin{figure}[h]
\centering
\includegraphics[scale=0.75]{CX_all_orthogonal_13tev.pdf}
\caption{\small  Cross section ratios ($\sigma_{BSM}/\sigma_{SM}$) in selected slices of parameter space. Left column: the plane of SM parameters, $\kappa_t : \kappa_\lambda$ (top), and the region allowing a Higgs contact interaction with gluons, $c_g : \kappa_\lambda$ (bottom). Middle column: planes spanned by the parameters describing non-vanishing one- and two-Higgs boson interactions with top quarks and with gluons, $\kappa_t : c_2$ (top) and $c_{2g} : c_g$ (bottom). Right column: comparison between gluon and top-quark interactions, $c_g : c_2$ (top) and $c_{2g}:c_2$ (bottom), for selected values of the other parameters; the relation $c_{2g}=-c_g$ is broken in the last graph.
\label{fig:cx}
}
\end{figure} 

%\newpage
\noindent
In general, BSM theories do not provide a unique prediction for the Higgs boson trilinear coupling. The current experimental limits on non-resonant Higgs pair production in the SM come from the study of the $\gamma\gamma\, b\bar{b}$ and $4b$ final states at 8 TeV by ATLAS~\cite{Aad:2014yja,Aad:2015uka}. Those limits are respectively $\sigma_{hh\to\gamma\gamma bb}^{SM} < 5.72$ fb (220 times the SM value) and $\sigma_{hh\to 4b}^{SM} < 202$ fb (56 times the SM value). Both results were derived by counting experiments and therefore without strong assumptions on the signal topology in the final state, other than the presence of two Higgs bosons. Considering the ATLAS SM results extended to all the parameter space, we find the $|\kappa_{\lambda}|$-only variation to be constrained in the region $|\kappa_{\lambda}| \simeq 15$~\footnote{The $\kappa_{\lambda}$ parameter is a multiplicative variation of a small value ($\lambda_{SM} \sim 0.13$), therefore an $O(10)$ variation would not affect the computational validity of the perturbative approach.} . Following a similar approach  the $c_2$ parameter can be constrained to $|c_2|<5$ at $95\%$ CL when $\kappa_{\lambda} = 1$ and $\kappa_{t} \subset [0.5\, , 2.5]$. 

A cursory look at the kinematics of the final state, as described in any of the already mentioned phenomenological references, suggests that different choices of the coupling parameters give rise to striking differences in the density functions of the kinematic observables. This convinces us of the need of a systematic approach to characterize the signal topology.

In order to retain generality of the results of our study to any final state of di-Higgs production, and invariant to further analysis cuts and/or analysis techniques, we study the event topology as it results from the production of the two Higgs bosons free from initial-state radiation effects and before the subsequent decays and final-state radiation effects. The study is performed with an extended sampling of parameter space points used to calculate the total cross section in last section; again, no generation cut is applied to the processes. For each studied point of the parameter space we generate 20,000 events of pp collisions at 13 TeV centre of mass energy.  These are sufficient for the task of understanding how the event kinematics varies as a function of the model parameters.

We are considering a $2\to 2$ process at leading order. The two Higgs bosons are produced with identical transverse momenta ($p_{T}^{h}$), and they are back-to-back in azimuth at this order (before a parton shower). The final state can then be completely defined by three kinematic variables, if we ignore the azimuthal angle of emission of the bosons. Furthermore, one of the three remaining variables can be used to isolate all the information related to the PDF of the colliding partons, which is irrelevant to the physics of the production process once one focuses on a specific initial state (the gluon-gluon fusion process). The variable factorizing out the PDF modelling can be taken as the magnitude of the boost of the centre of mass frame as seen in the laboratory frame. 

The two remaining variables, which provide direct information on the physics of GF di-Higgs production, can be chosen to be the invariant mass of the di-Higgs system ($m_{hh}$) and the modulus of the cosine of the  polar angle of one Higgs boson with respect to the beam axis ($|cos\theta^*|$). 
Since we are using parton level information, this last variable is equivalent to the polar angle in the Collins-Soper frame ($|cos\theta^*_{CS}|$)~\cite{PhysRevD.16.2219}, which is commonly used in experimental analysis. In this work we will rely on $m_{hh}$ and $|cos\theta^*|$ to characterize the final state kinematics produced by different choices of the value of anomalous Higgs (self-) coupling parameters.

